On the Fast Magnetic Rotator Regime of Stellar Winds

Aims: We study the acceleration of the stellar winds of rapidly rotating low mass stars and the transition between the slow magnetic rotator and fast magnetic rotator regimes. We aim to understand the properties of stellar winds in the fast magnetic rotator regime and the effects of magneto-centrifugal forces on wind speeds and mass loss rates. Methods: We extend the solar wind model of Johnstone et al. (2015b) to 1D magnetohydrodynamic (MHD) simulations of the winds of rotating stars. We test two assumptions for how to scale the wind temperature to other stars and assume the mass loss rate scales as Mdot ~ Rstar^2 OmegaStar^1.33 Mstar^-3.36, in the unsaturated regime, as estimated by Johnstone et al. (2015a). Results: For 1.0 Msun stars, the winds can be accelerated to several thousand km/s, and the effects of magneto-centrifugal forces are much weaker for lower mass stars. We find that the different assumptions for how to scale the wind temperature to other stars lead to significantly different mass loss rates for the rapid rotators. If we assume a constant temperature, the mass loss rates of solar mass stars do not saturate at rapid rotation, which we show to be inconsistent with observed rotational evolution. If we assume the wind temperatures scale positively with rotation, the mass loss rates are only influenced significantly at rotation rates above 75 OmegaSun. We suggest that models with increasing wind speed for more rapid rotators are preferable to those that assume a constant wind speed. If this conclusion is confirmed by more sophisticated wind modelling. it might provide an interesting observational constraint on the properties of stellar winds.

==> Journals.tex <==
\newcommand{\aj}{{AJ}}			
\newcommand{\araa}{{Ann.\ Rev.\ Astron.\ Astrophys.}}		
\newcommand{\apj}{{ApJ}}			
\newcommand{\apjl}{{ApJ Lett.}}		
\newcommand{\apjs}{{ApJS}}		
\newcommand{\apss}{{Ap\&SS}}		
\newcommand{\aap}{{A\&A.}}		
\newcommand{\aapr}{{A\&A~Rev.}}		
\newcommand{\aaps}{{A\&AS}}		
\newcommand{\an}{{AN}}			
\newcommand{\azh}{{AZh}}			
\newcommand{\baas}{{BAAS}}		
\newcommand{\BAIC}{{Bull.\ Astron.\ Inst.\ Czech.}}		
\newcommand{\jrasc}{{JRASC}}		
\newcommand{\memras}{{MmRAS}}		
\newcommand{\mnras}{{MNRAS}}		
\newcommand{\pra}{{Phys.~Rev.~A}}	
\newcommand{\prb}{{Phys.~Rev.~B}}	
\newcommand{\prc}{{Phys.~Rev.~C}}	
\newcommand{\prd}{{Phys.~Rev.~D}}	
\newcommand{\pre}{{Phys.~Rev.~E}}	
\newcommand{\prl}{{Phys.~Rev.~Lett.}}	
\newcommand{\pasp}{{PASP}}		
\newcommand{\pasj}{{PASJ}}		
\newcommand{\qjras}{{QJRAS}}		
\newcommand{\skytel}{{S\&T}}		
\newcommand{\solphys}{{Solar~Phys.}}	
\newcommand{\sovast}{{Soviet~Ast.}}	
\newcommand{\ssr}{{Space~Sci.~Rev.}}	
\newcommand{\zap}{{ZAp}}			
\newcommand{\nat}{{Nature}}		
\newcommand{\iaucirc}{{IAU~Circ.}}
\newcommand{\aplett}{{Astrophys.~Lett.}}
\newcommand{\apspr}{{Astrophys.~Space~Phys.~Res.}}
\newcommand{\bain}{{Bull.~Astron.~Inst.~Netherlands}}
\newcommand{\fcp}{{Fund.~Cosmic~Phys.}}
\newcommand{\gca}{{Geochim.~Cosmochim.~Acta}}
\newcommand{\grl}{{Geophys.~Res.~Lett.}}
\newcommand{\GAFD}{{Geophys.~Astrophys.~Fluid~Dyn.}}
\newcommand{\jcp}{{J.~Chem.~Phys.}}	
\newcommand{\jgr}{{J.~Geophys.~Res.}}	
\newcommand{\jqsrt}{{J.~Quant.~Spec.~Radiat.~Transf.}}
\newcommand{\memsai}{{Mem.~Soc.~Astron.~Italiana}}
\newcommand{\nphysa}{{Nucl.~Phys.~A}}
\newcommand{\physrep}{{Phys.~Rep.}}
\newcommand{\physscr}{{Phys.~Scr}}
\newcommand{\planss}{{Planet.~Space~Sci.}}
\newcommand{\procspie}{{Proc.~SPIE}}
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao
